Semi-supervised Contrastive Regression for Estimation of Eye Gaze

With the escalated demand of human-machine interfaces for intelligent systems, development of gaze controlled system have become a necessity. Gaze, being the non-intrusive form of human interaction, is one of the best suited approach. Appearance based deep learning models are the most widely used for gaze estimation. But the performance of these models is entirely influenced by the size of labeled gaze dataset and in effect affects generalization in performance. This paper aims to develop a semi-supervised contrastive learning framework for estimation of gaze direction. With a small labeled gaze dataset, the framework is able to find a generalized solution even for unseen face images. In this paper, we have proposed a new contrastive loss paradigm that maximizes the similarity agreement between similar images and at the same time reduces the redundancy in embedding representations. Our contrastive regression framework shows good performance in comparison to several state of the art contrastive learning techniques used for gaze estimation.

==> refbank_gaze.tex <==
%%%%Applications

@article{konrad2020gaze,
  title={Gaze-contingent ocular parallax rendering for virtual reality},
  author={Konrad, Robert and Angelopoulos, Anastasios and Wetzstein, Gordon},
  journal={ACM Transactions on Graphics (TOG)},
  volume={39},
  number={2},
  pages={1--12},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@inproceedings{gerber2020self,
  title={Self-interruptions of non-driving related tasks in automated vehicles: Mobile vs head-up display},
  author={Gerber, Michael A and Schroeter, Ronald and Xiaomeng, Li and Elhenawy, Mohammed},
  booktitle={Proceedings of the 2020 CHI Conference on Human Factors in Computing Systems},
  pages={1--9},
  year={2020}
}

@article{ferrier2022measuring,
  title={Measuring the Quality of Learning in a Human--Robot Collaboration: A Study of Laparoscopic Surgery},
  author={Ferrier-Barbut, El{\'e}onore and Gauthier, Philippe and Luengo, Vanda and Canlorbe, Geoffroy and Vitrani, Marie-Aude},
  journal={ACM Transactions on Human-Robot Interaction (THRI)},
  volume={11},
  number={3},
  pages={1--20},
  year={2022},
  publisher={ACM New York, NY}
}

%%%%%%%%%%features
@article{rattarom2019model,
  title={Model Construction and Validation in Low-cost Interpolation-Based Gaze Tracking System.},
  author={Rattarom, Suwitchaya and Uttama, Surapong and Aunsri, Nattapol},
  journal={Engineering Letters},
  volume={27},
  number={1},
  year={2019}
}

@inproceedings{yilmaz2016local,
  title={Local binary pattern histogram features for on-screen eye-gaze direction estimation and a comparison of appearance based methods},
  author={Yilmaz, Cagatay Murat and Kose, Cemal},
  booktitle={2016 39th International Conference on Telecommunications and Signal Processing (TSP)},
  pages={693--696},
  year={2016},
  organization={IEEE}
}

@article{aunsri2022novel,
	title={Novel eye-based features for head pose-free gaze estimation with web camera: New model and low-cost device},
	author={Aunsri, Nattapol and Rattarom, Suwitchaya},
	journal={Ain Shams Engineering Journal},
	volume={13},
	number={5},
	pages={101731},
	year={2022},
	publisher={Elsevier}
}

%%survey
@article{pathirana2022eye,
	title={Eye gaze estimation: A survey on deep learning-based approaches},
	author={Pathirana, Primesh and Senarath, Shashimal and Meedeniya, Dulani and Jayarathna, Sampath},
	journal={Expert Systems with Applications},
	volume={199},
	pages={116894},
	year={2022},
	publisher={Elsevier}
}

@article{cheng2021appearance,
	title={Appearance-based gaze estimation with deep learning: A review and benchmark},
	author={Cheng, Yihua and Wang, Haofei and Bao, Yiwei and Lu, Feng},
	journal={arXiv preprint arXiv:2104.12668},
	year={2021}
}

@article{lemley2019convolutional,
	title={Convolutional neural network implementation for eye-gaze estimation on low-quality consumer imaging systems},
	author={Lemley, Joseph and Kar, Anuradha and Drimbarean, Alexandru and Corcoran, Peter},
	journal={IEEE Transactions on Consumer Electronics},
	volume={65},
	number={2},
	pages={179--187},
	year={2019},
	publisher={IEEE}
}

%%resnet

@article{kanade2021convolutional,
  title={Convolutional neural networks (CNN) based eye-gaze tracking system using machine learning algorithm},
  author={Kanade, Prakash and David, Fortune and Kanade, Sunay},
  journal={European Journal of Electrical Engineering and Computer Science},
  volume={5},
  number={2},
  pages={36--40},
  year={2021}
}

@article{zhu2022complementary,
  title={A Complementary Dual-branch Network for Appearance-based Gaze Estimation from Low-resolution Facial Image},
  author={Zhu, Zhesi and Zhang, Dong and Chi, Cailong and Li, Ming and Lee, Dah-Jye},
  journal={IEEE Transactions on Cognitive and Developmental Systems},
  year={2022},
  publisher={IEEE}
}

@inproceedings{chong2020detecting,
	title={Detecting attended visual targets in video},
	author={Chong, Eunji and Wang, Yongxin and Ruiz, Nataniel and Rehg, James M},
	booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
	pages={5396--5406},
	year={2020}
}

@inproceedings{bernard2021eye,
	title={Eye-Gaze Estimation using a Deep Capsule-based Regression Network},
	author={Bernard, Vivien and Wannous, Hazem and Vandeborre, Jean-Philippe},
	booktitle={2021 International Conference on Content-Based Multimedia Indexing (CBMI)},
	pages={1--6},
	year={2021},
	organization={IEEE}
}

@inproceedings{mahanama2020gaze,
	title={Gaze-Net: Appearance-based gaze estimation using capsule networks},
	author={Mahanama, Bhanuka and Jayawardana, Yasith and Jayarathna, Sampath},
	booktitle={Proceedings of the 11th augmented human international conference},
	pages={1--4},
	year={2020}
}

%%%%%%%%%%%contrastive

@inproceedings{crawford2019spatially,
  title={Spatially invariant unsupervised object detection with convolutional neural networks},
  author={Crawford, Eric and Pineau, Joelle},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  number={01},
  pages={3412--3420},
  year={2019}
}

@inproceedings{chen2020simple,
  title={A simple framework for contrastive learning of visual representations},
  author={Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle={International conference on machine learning},
  pages={1597--1607},
  year={2020},
  organization={PMLR}
}

@article{grill2020bootstrap,
  title={Bootstrap your own latent-a new approach to self-supervised learning},
  author={Grill, Jean-Bastien and Strub, Florian and Altch{\'e}, Florent and Tallec, Corentin and Richemond, Pierre and Buchatskaya, Elena and Doersch, Carl and Avila Pires, Bernardo and Guo, Zhaohan and Gheshlaghi Azar, Mohammad and others},
  journal={Advances in neural information processing systems},
  volume={33},
  pages={21271--21284},
  year={2020}
}

@inproceedings{zbontar2021barlow,
  title={Barlow twins: Self-supervised learning via redundancy reduction},
  author={Zbontar, Jure and Jing, Li and Misra, Ishan and LeCun, Yann and Deny, St{\'e}phane},
  booktitle={International Conference on Machine Learning},
  pages={12310--12320},
  year={2021},
  organization={PMLR}
}

@inproceedings{wang2022contrastive,
  title={Contrastive regression for domain adaptation on gaze estimation},
  author={Wang, Yaoming and Jiang, Yangzhou and Li, Jin and Ni, Bingbing and Dai, Wenrui and Li, Chenglin and Xiong, Hongkai and Li, Teng},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={19376--19385},
  year={2022}
}


@inproceedings{chen2018encoder,
  title={Encoder-decoder with atrous separable convolution for semantic image segmentation},
  author={Chen, Liang-Chieh and Zhu, Yukun and Papandreou, George and Schroff, Florian and Adam, Hartwig},
  booktitle={Proceedings of the European conference on computer vision (ECCV)},
  pages={801--818},
  year={2018}
}

%%%Dataset
@inproceedings{zhang2020eth,
  title={Eth-xgaze: A large scale dataset for gaze estimation under extreme head pose and gaze variation},
  author={Zhang, Xucong and Park, Seonwook and Beeler, Thabo and Bradley, Derek and Tang, Siyu and Hilliges, Otmar},
  booktitle={Computer Vision--ECCV 2020: 16th European Conference, Glasgow, UK, August 23--28, 2020, Proceedings, Part V 16},
  pages={365--381},
  year={2020},
  organization={Springer}
}























